Learn Beyond The Answer: Training Language Models with Reflection for Mathematical Reasoning

Supervised fine-tuning enhances the problem-solving abilities of language models across various mathematical reasoning tasks. To maximize such benefits, existing research focuses on broadening the training set with various data augmentation techniques, which is effective for standard single-round question-answering settings. Our work introduces a novel technique aimed at cultivating a deeper understanding of the training problems at hand, enhancing performance not only in standard settings but also in more complex scenarios that require reflective thinking. Specifically, we propose reflective augmentation, a method that embeds problem reflection into each training instance. It trains the model to consider alternative perspectives and engage with abstractions and analogies, thereby fostering a thorough comprehension through reflective reasoning. Extensive experiments validate the achievement of our aim, underscoring the unique advantages of our method and its complementary nature relative to existing augmentation techniques.

==> latex/Sections/1_intro_alternative.tex <==
\begin{figure*}[ht]
    
        \centering
        \includegraphics[width=0.85\textwidth]{latex/Figures/intro_illustration_revised.pdf}
        \caption{Illustration of different data augmentation methods in reasoning learning. Reflective augmentation is orthogonal to and can be seamlessly integrated with previous augmentation methods.}
        \label{fig:intro_illustration}
    
\end{figure*}

\begin{figure*}[ht]
    \centering

        \includegraphics[width=0.95\textwidth]{latex/Figures/Intro_example.pdf}
        \caption{Top: Reflective content is appended to the original solution for data augmentation. It includes {\color{ForestGreen}reflection on the problem}, {\color{Red}reflection on the solution}, and {\color{CornflowerBlue}reflection on the related concepts}. Bottom: The student gains a more comprehensive understanding of the related knowledge after learning from the reflection data (right), rather than merely memorizing the original solution (left).}
        \label{fig:intro_example}

\end{figure*}
    


Reasoning is a cornerstone of human intelligence, which makes it pivotal for language models (LMs) to emulate before being regarded as human-like AI assistants. The mastery of reasoning extends LMs' capabilities beyond mere language imitation to broader applications such as solving mathematical problems~\cite{chain-of-thought,zero-shot-cot,mammoth}, coding~\cite{PAL,wizardcoder}, logical thinking~\cite{are-llm-good-logical-reasoners,logic-lm}, etc. However, the limited quantity and quality of human-annotated data for reasoning learning restricts the potential for LMs to advance their reasoning abilities~\cite{Xwin,reformat-alignment}.

To address this limitation, data augmentation emerges as a crucial strategy to enhance the reasoning performance of LMs. The most straightforward method is data scaling, where common approaches are mainly categorized into \textit{question augmentation} (Figure~\ref{fig:intro_illustration}b, \citealp{wizardmath,metamath,orcamath,Xwin}) -- constructing additional questions based on existing ones -- and \textit{answer augmentation} (Figure~\ref{fig:intro_illustration}c, \citealp{rft,mugglemath,metamath}), which samples the solution multiple times for each problem to increase diversity. Although these methods do improve the model's reasoning performance, the augmentation rules must be meticulously designed to balance data quality and diversity~\cite{mathcoder,mathscale}. Moreover, integrating various types of augmented data does not always yield further improvements~\cite{metamath}, and consistently employing the same augmentation strategy may eventually lead to training saturation, where performance gains diminish~\cite{rft,mugglemath}.

Besides data scaling, another augmentation strategy is \textit{answer enrichment} (Figure~\ref{fig:intro_illustration}d), which targets the quality deficits of human-annotated data. This method refines the original answers to better align with human cognitive processes and fills logical gaps to enhance quality~\cite{reformat-alignment,enrichmath}. Such an approach, though also effective, is highly dependent on the original answer's line of thought, constraining its scope to augmenting within pre-existing reasoning patterns. 
% on the content of the original answer, making its augmentation perspective restricted to the original chain of thought.

% To augment LMs' reasoning abilities, the construction of high-quality training data is considered an essential step. Following such intuition, the majority of previous efforts have focused on expanding the size of training set by including more diverse problems and solutions. Such approaches can be mainly categorized into \textit{question augmentation}, which collects new questions based on existing ones, and \textit{answer augmentation}, which samples the solution multiple times for each problem to increase diversity.

In order to complement the limitations of existing augmentation dimensions, in this work, we explore an orthogonal and unexplored direction: \textit{reflective augmentation} (Figure~\ref{fig:intro_illustration}e). Reflection is a process that humans use to critically analyze and evaluate their problem-solving procedure, which encompasses comprehending underlying concepts, exploring various problem-solving strategies, and applying these insights to related problems~\cite{alternative-1,followup-1}. Drawing from these cognitive patterns, our reflective augmentation appends reflective content to the original solution. Specifically, for a given problem, the model is trained to generate both the original solution and the reflective content in a single pass. An example is shown in Figure~\ref{fig:intro_example}, where the reflective content provides a deeper understanding of the problem and its solution. This method not only strengthens the model's grasp of related mathematical knowledge but also discourages rote memorization of solutions, thereby helping it solve relevant problems during inference.
% The additional training on reflective content not only helps the modeling of the original solution but also does so without impacting the efficiency of decoding during inference.
The benefits of this approach are three-fold: (1) it deepens the model's understanding of the problem by reiterating the critical reasoning steps and knowledge from a reflective perspective; (2) it develops the model's capacity for reflective thinking, vital for handling more complex reasoning scenarios; (3) it is orthogonal to existing augmentation strategies, enabling their seamless integration to further improve the training of LMs.

% While the expansion of training set enhances LMs' performance across diverse problem types, an equally important direction -- the thorough understanding of individual problems -- is often overlooked. In human learning, besides learning more individual problems, another common cognitive strategy involves deepening the understanding of a problem through reflective thinking that extends beyond the initial solution. This reflection may encompass comprehending underlying concepts, exploring various problem-solving strategies, and applying these insights to related problems. Such reflective processes create a rich context around a problem, enhancing understanding and the associated problem-solving strategies.

% In light of these human cognitive patterns, our approach integrates reflective thinking into the training data for LMs. We enrich training examples by appending reflective data to original solutions. Specifically, we train LMs to generate alternative problem-solving strategies and related follow-up problems while keeping the original solution intact, as illustrated in Figure~\ref{fig:intro}. Such an approach provides a comprehensive context for each training problem, which not only helps strengthen the model's understanding of each problem but also bolsters the acquisition of related reasoning skills.

To verify the aforementioned benefits in reasoning learning of LMs, we conduct experiments on training LMs with reflective augmentation data across multiple reasoning scenarios, including mathematical reasoning and code generation datasets. Our results indicate that training with reflective data significantly boosts LMs' reasoning capabilities compared to standard fine-tuning recipes. Particularly, our training strategy greatly improves LMs' performance in reasoning tasks that require reflective thinking, where traditional augmentation methods fall short. Moreover, this strategy integrates seamlessly with other augmentation approaches, achieving greater improvements than the repeated use of a single method. This confirms that our reflective training strategy is both orthogonal to and a valuable addition to existing methods. 

In summary, our main contributions include:
\begin{itemize}
[noitemsep,topsep=1pt,parsep=1pt,partopsep=0pt]
\item We delve into the use of reflective augmentation data in training LMs for reasoning tasks. By training LMs to continue generating reflective content following the original solution, we aim to deepen the model's understanding of each problem and foster their reflective thinking abilities.
\item Our extensive experiments demonstrate that this training approach substantially enhances LMs' reasoning capabilities, especially in scenarios that demand reflective thinking.
\item Besides, we prove that our method not only stands orthogonal to but also enhances existing training augmentation methods. This synergy allows for a more substantial improvement in performance.

\end{itemize}
